On minimizers of the maximal distance functional for a planar convex closed smooth curve

Fix a compact $M \subset \mathbb{R}^2$ and $r>0$. A minimizer of the maximal distance functional is a connected set $\Sigma$ of the minimal length, such that \[ max_{y \in M} dist(y,\Sigma) \leq r. \] The problem of finding maximal distance minimizers is connected to the Steiner tree problem. In this paper we consider the case of a convex closed curve $M$, with the minimal radius of curvature greater than $r$ (it implies that $M$ is smooth). The first part is devoted to statements on structure of $\Sigma$: we show that the closure of an arbitrary connected component of $B_r(M) \cap \Sigma$ is a local Steiner tree which connects no more than five vertices. In the second part we "derive in the picture". Assume that the left and right neighborhoods of $y \in M$ are contained in $r$-neighborhoods of different points $x_1$, $x_2 \in \Sigma$. We write conditions on the behavior of $\Sigma$ in the neighborhoods of $x_1$ and $x_2$ under the assumption by moving $y$ along $M$.

==> pictures/rus/MMrNNr.tex <==
\begin{figure}[h]
    \centering
    \begin{tikzpicture}
    \fill[lightgray!50] plot [smooth cycle, tension=1] coordinates 
        {(0,0) (0,3) (4,3) (4.5, 0)};
    \draw[very thick] plot [smooth cycle, tension=1] coordinates 
        {(0,0) (0,3) (4,3) (4.5, 0)};
    \draw[very thick, pattern=dots] plot [smooth cycle, tension=1] coordinates 
        {(0.7,0.7) (0.7,2.3) (3.3,2.3) (3.8, 0.7)};
    \draw[<->] (2.2,-0.5) -- (2.2,0.3);
        
    \node[above] at (2, 3.6) {$M$};
    \node[above] at (2, 2.6) {$M_r$};
    \node[right] at (2.2, -0.1) {$r$};
    
    \draw[fill = lightgray!50] (6,1) rectangle (6.5,1.5);
    \draw[pattern=dots] (6,0) rectangle (6.5,0.5);
    \node[right] at (6.5, 1.25) {$N$};
    \node[right] at (6.5, 0.25) {$N_r$};
\end{tikzpicture}

    \caption{Определение $N$, $M_r$ и $N_r$}
    \label{MMrNNr}
\end{figure}

==> pictures/rus/case12.tex <==
\begin{figure}[h]
    \centering
    %
    %
    \hfill
    %
    %
    \begin{tikzpicture}[scale=1.2]
    \def\eps{\varepsilon}
    
    \clip(-5,-3) rectangle (1,2);
    
    \draw[very thick] plot [smooth, tension=1] coordinates
        {(-5, 0) (0, 1) (5, 0)};
        
    \draw (-5, 1.01) -- (5, 1.01);
    \draw[dotted] (-2,1) arc (180:360:2);
    
    \draw[dashed] (0, 1) -- (-1.6, -.2);
    \draw[very thick, blue] (-4, -2) -- (-1.6, -.2);
    
    %\draw[thick, dotted] (-4, -2) -- (-4, 1);
    %\draw[thin] (-4, .8) -- (-3.8, .8) -- (-3.8, 1);
    
    \draw (-.7, 1) arc (180 : 216.87 : 0.7);
    \draw (-.75, 1) arc (180 : 216.87 : 0.75);
    
    \node[left] at (-.7, 0.7) {$\alpha$}; 
    
    %\draw [decorate , decoration={brace,amplitude=3pt},
   %         xshift=-4pt,yshift=0pt]
    %    (-4, -1.98) -- (-4, .98) node [midway,xshift=-0.5cm] {$h$};
        
    %\draw [decorate , decoration={brace,mirror, amplitude=3pt},      
    %        xshift=0pt,yshift=4pt]
     %   (-0.02, 1) -- (-3.98, 1) node [midway,yshift=0.5cm] {$a$};
    \draw [decorate , decoration={brace,mirror, amplitude=3pt},      
            xshift=0pt,yshift=4pt]
        (0.68, 1) -- (0.02, 1) node [midway,yshift=0.5cm] {$\eps$};
    
    \fill (0,1) circle (1.5pt)
        node[below] {{\small $y(x)$}};
        
    \fill[blue] (-1.6, -.2) circle (1.5pt);
    \node[above] at (-1.6, -.1) {$x$};
    
    \fill[blue] (-4, -2) circle (0pt) 
        node[below, black] {$z$};
        
    \fill (0.7, .97) circle (1.5pt)
        node[below] {{\small $y(x_\varepsilon)$}};

    
\end{tikzpicture}
%
%
%
\hfill
%
%
%
\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=1cm,y=1cm,scale=1.2]
\clip(-4.5, -.8) rectangle (2., 4.2);


\draw [very thick, shift={(-0.12513485800546506,-26.677521852562677)}]  plot[domain=1.3015317814364376:1.81024140245113,variable=\t]({1*30.392666753240377*cos(\t r)+0*30.392666753240377*sin(\t r)},{0*30.392666753240377*cos(\t r)+1*30.392666753240377*sin(\t r)});

\draw [dotted] (1.6662008271652229,3.6623085496751884) circle (2.7202892533708605cm);
\draw [dotted] (-0.4727808370220571,3.7131565644584974) circle (2.7202892533708605cm);

\draw [very thick, blue] (-3.783717507507988,1.056029328176248)-- (-1.530653918438071,1.2069885402389755);
\draw [very thick, blue] (-1.530653918438071,1.2069885402389755)-- (-0.06721948175656989,-0.5127334924261615);
\draw [very thick, blue, dashed] (-0.20613901407786517,1.6889061221660897)-- (-0.06721948175656989,-0.5127334924261615);
\draw [very thick, blue, dashed] (-0.20613901407786517,1.6889061221660897)-- (-3.783717507507988,1.056029328176248);
\draw [] (-1.1576901280692398,2.0905632733845843)-- (-0.06721948175656989,-0.5127334924261615);
\draw [] (-1.1576901280692398,2.0905632733845843)-- (-3.783717507507988,1.056029328176248);
% УГЛЫ

\draw [shift={(-1.1576901280692398,2.0905632733845843)}] (-67.27213315390254:0.3003568321075131) arc (-67.27213315390254:-22.884987621529085:0.3003568321075131);
\draw[] (-0.9721088011312526,1.9044723323699622) -- (-0.9190855648632562,1.8513034920800702);

\draw [shift={(-1.530653918438071,1.2069885402389755)}] (-112.88498762152909:0.3003568321075131) arc (-112.88498762152909:-49.60316378273691:0.3003568321075131);

\draw [shift={(-1.530653918438071,1.2069885402389755)}] (-112.88498762152909:0.23527951848421863) arc (-112.88498762152909:-49.60316378273691:0.23527951848421863);

\draw [shift={(-1.530653918438071,1.2069885402389755)}] (-176.16681146032127:0.35041630412543195) arc (-176.16681146032127:-112.88498762152908:0.35041630412543195);

\draw [shift={(-1.530653918438071,1.2069885402389755)}] (-176.16681146032127:0.28533899050213746) arc (-176.16681146032127:-112.88498762152908:0.28533899050213746);

\draw [shift={(-1.1576901280692398,2.0905632733845843)}] (-67.27213315390254:0.3003568321075131) arc (-67.27213315390254:-22.884987621529085:0.3003568321075131);

\draw [shift={(-0.4727808370220571,3.7131565644584974)}] (-179.34460895105994:0.35041630412543195) arc (-179.34460895105994:-112.88498762152909:0.35041630412543195) ;

\draw [shift={(-1.1576901280692398,2.0905632733845843)}] (157.1150123784709:0.3003568321075131) arc (157.1150123784709:201.50215791084437:0.3003568321075131);


\draw [dashed] (-0.4727808370220571,3.7131565644584974)-- (-2.0483888830006287,-0.019558231771048984);
%\draw [] (-3.805924672756144,3.67502796344221)-- (3.409048634201412,3.7575617069953324);
\draw [dashed] (-3.8848543096703176,3.2417205575080885)-- (2.4644358241962365,0.5616356414899564);
\draw [dashed] (2.3181285497377746,-0.41761257587217493)-- (-4.04973666644738,2.270313027354491);
%\draw [shift={(-1.1576901280692398,2.0905632733845843)}] (157.1150123784709:0.3003568321075131) arc (157.1150123784709:201.50215791084437:0.3003568321075131);
\draw[] (-1.4204832205471947,2.093734673965504) -- (-1.4955669612551816,2.094640788417195);
\fill [blue] (-1.530653918438071,1.2069885402389755) circle (1pt);
\node[black, right] at (-1.5 ,1.3) {$x$};
\fill [blue] (-0.06721948175656989,-0.5127334924261615) circle (1pt)
    node[black, right] {$z_{1}$};
\fill [blue] (-3.783717507507988,1.056029328176248) circle (1pt)
    node[black, left] {$z_{2}$};
\fill [black] (-0.4727808370220571,3.7131565644584974) circle (1pt)
    node[above] {$y(x)$};
\fill [black] (1.6662008271652229,3.6623085496751884) circle (1pt)
    node[below] {$y(x_{\varepsilon})$};
\fill [blue] (-0.20613901407786517,1.6889061221660897) circle (1pt)
    node[black, above right] {$x_\varepsilon$};
\fill [black] (-1.1576901280692398,2.0905632733845843) circle (1pt);
\fill [white] (-1.1,2.25) circle (3pt);
\node[above] at (-1.05,2.1) {$x_{new}$};
\draw[] (-0.8,1.8) node {$\gamma$};
\draw[] (-0.95,3.5547777778793734) node {$\alpha$};
\draw[] (-1.5, 0.7) node {$\beta$};
\end{tikzpicture}
%
%
%
\hfill\phantom{}
    \caption{Первый и второй случаи дифференцирования}
    \label{case12}
\end{figure}

==> pictures/rus/case34.tex <==
\begin{figure}[h]
    \centering
    %
    %
    %
    %
    \hfill
    %
    %
    %
    \begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=1cm,y=1cm]
        \clip(-3.5,-4) rectangle (6.2,3);
        
        
        \draw [->, dashed] (0.5107776365566263,-3.1910707849251336) -- (0.4924206181982182,2.411863460903201) node[right]{$Y$};
        
        \draw [->, dashed] (-3.372996196881047,-1.7512031984129917)-- (5.640695451173274,-1.7216714395522534) node[below]{$X$};
        
        %\draw [shift={(3.4322447318135465,-1.7289070358702208)}]  (-179.81228123213836:0.5413606833758918) arc (-179.81228123213836:-163.71276489579233:0.5413606833758918);
        %\draw [shift={(-2.420207676157121,-1.74808155614499)}] (0.18771876786164332:1.2180615375957566) arc (0.18771876786164332:7.109991463141681:1.2180615375957566);
        %\draw (-1.255265041923725,-1.6737922660197848) -- (-1.153965682425169,-1.6673323277480274);
        %\draw [shift={(0.4963164562849324,1.2227746771979466)},dash pattern=on 2pt off 1pt] (-57.29233279583929:0.5413606833758919) arc (-57.29233279583929:0.18771876786163338:0.5413606833758919);
        
        \draw [shift={(3.4322447318135465,-1.7289070358702208)}] (134.8466944428081:0.4060205125319189) arc (134.8466944428081:180.18771876786164:0.4060205125319189);
        \draw [shift={(3.4322447318135465,-1.7289070358702208)}] (134.8466944428081:0.3180494014833365) arc (134.8466944428081:180.18771876786164:0.3180494014833365);
        \draw [shift={(5.6375557440695685,-0.7430070915455227)}] (174.33339161087738:0.7443709396418513) arc (174.33339161087738:187.10999146314168:0.7443709396418513);
        \draw [shift={(5.6375557440695685,-0.7430070915455227)}] (174.33339161087738:0.6563998285932688) arc (174.33339161087738:187.10999146314168:0.6563998285932688);
        \draw [shift={(5.6375557440695685,-0.7430070915455227)}] (174.33339161087738:0.5684287175446864) arc (174.33339161087738:187.10999146314168:0.5684287175446864);
        
        \draw [shift={(0.4963164562849324,1.2227746771979466)}] (-179.81228123213836:0.47369059795390545) arc (-179.81228123213836:-134.47125690708478:0.47369059795390545);
        \draw [shift={(0.4963164562849324,1.2227746771979466)}] (-179.81228123213836:0.385719486905323) arc (-179.81228123213836:-134.47125690708478:0.385719486905323);
        \draw [shift={(-2.420207676157124,-1.7480815561449892)}] (7.109991463141661:0.7443709396418514) arc
        (7.109991463141661:19.886591315406243:0.7443709396418514);
        \draw [shift={(-2.420207676157124,-1.7480815561449892)}] (7.109991463141661:0.656399828593269) arc (7.109991463141661:19.886591315406243:0.656399828593269);
        \draw [shift={(-2.420207676157124,-1.7480815561449892)}] (7.109991463141661:0.5684287175446865) arc (7.109991463141661:19.886591315406243:0.5684287175446865);
        \draw [shift={(-2.420207676157124,-1.7480815561449892)}] (0.1877187678616431:0.40602051253191895) arc (0.1877187678616431:45.5287430929152:0.40602051253191895);
        \draw [shift={(-2.420207676157124,-1.7480815561449892)}] (0.1877187678616431:0.3180494014833365) arc (0.1877187678616431:45.5287430929152:0.3180494014833365);
        
        
        \draw [rotate around={0.18771876786163075:(0.4904347574391314,3.0179884337769978)},very thick] (0.4904347574391314,3.0179884337769978) ellipse (7.535706036941022cm and 5.161556748282821cm);
        
        \draw [dotted] (-2.420207676157121,-1.74808155614499) circle (4.163183850649577cm);
        \draw [dotted] (3.4322447318135465,-1.7289070358702208) circle (4.163183850649577cm);
        
        \draw [] (-2.420207676157121,-1.74808155614499)-- (3.4322447318135465,-1.7289070358702208);
        \draw [] (5.6375557440695685,-0.7430070915455227)-- (3.4322447318135465,-1.7289070358702208) 
            node[above, pos=0.75]{$\varepsilon$};
        \draw [] (0.4963164562849324,1.2227746771979437)-- (-2.420207676157121,-1.74808155614499) 
            node[above left, pos=0.5]{$r$};
        \draw [] (0.4963164562849324,1.2227746771979437)-- (3.4322447318135465,-1.7289070358702208) 
            node[above right, pos=0.4]{$r$};
        \draw [] (-2.420207676157121,-1.74808155614499)-- (5.6375557440695685,-0.7430070915455227);
        \draw [] (1.4947161910399636,-0.3319350635955565)-- (-2.420207676157121,-1.74808155614499) 
            node[above, pos=0.4]{$r$};
        \draw [] (1.4947161910399636,-0.3319350635955565)-- (5.6375557440695685,-0.7430070915455227) 
            node[above, pos=0.5]{$r$};
        \draw [] (0.4963164562849324,1.2227746771979437)-- (1.4947161910399636,-0.3319350635955565);
        
        \draw [] (-2.9430712147632248,-3.591638176924038)-- (6.270436727691272,-0.8996479592514579);
        \draw [dashed] (-1.3967761861461803,1.2165722955767182)-- (2.8257031352740394,1.2304064986960972);
        
        \fill [black] (-2.420207676157121,-1.74808155614499) circle (2pt) 
            node[below] {$y_1(x)$};
        \fill [black] (3.4322447318135465,-1.7289070358702208) circle (2pt)  
            node[below]{$y_2(x)$};
        \fill [white] (0.72,1.42) circle (4pt);
        \fill [blue] (0.4963164562849324,1.2227746771979437) circle (2pt)
            node[black,above right]{$x$};
        \fill[white] (6,-0.4430070915455227) circle (8pt);
        \fill [black] (5.6375557440695685,-0.7430070915455227) circle (2pt)
            node[above]{$y_2(x_\varepsilon)$};
        
        \node[left] at (3.1210194681658792,-1.5143221866701352) {$\alpha$};
        \fill [blue] (1.4947161910399636,-0.3319350635955565) circle (2pt);
        \node[below] at (1.3947161910399636,-0.4319350635955565)
            {$x_\varepsilon$};
        \fill[white] (2.666203058140344,-1.7903426992020517) circle (3pt);
        \node at (2.666203058140344,-1.7503426992020517) {$\delta$};
        \node[left] at (4.780441689137528,-0.7534852641126851) {$\alpha_\varepsilon$};
        \fill[white] (-0.9, -1.5739550067212016) circle (3pt);
        \node[right] at (-1.175206169685229, -1.5839550067212016) {$\Delta$};
        %\node at (1.95,0.95) {\small$\frac \pi2 - \alpha + o(1)$};
    
    \end{tikzpicture}
%
%
%
%
%
    \hfill
%
%
%
%
%
    \begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=1cm,y=1cm, scale=1.5]
        \clip(-1, -1.5) rectangle (3,3);
        
        
        \draw [->, dashed] (0.5107776365566263,-3.1910707849251336) -- (0.4924206181982182,2.811863460903201) node[right]{$Y$};
        
        % \draw [->, dashed] (-3.372996196881047,-1.7512031984129917)-- (5.640695451173274,-1.7216714395522534) node[below]{$X$};
        
        % %\draw [shift={(3.4322447318135465,-1.7289070358702208)}]  (-179.81228123213836:0.5413606833758918) arc (-179.81228123213836:-163.71276489579233:0.5413606833758918);
        % %\draw [shift={(-2.420207676157121,-1.74808155614499)}] (0.18771876786164332:1.2180615375957566) arc (0.18771876786164332:7.109991463141681:1.2180615375957566);
        % %\draw (-1.255265041923725,-1.6737922660197848) -- (-1.153965682425169,-1.6673323277480274);
        
        
        \draw [shift={(0.4963164562849324,1.2227746771979466)}] (-57.29233279583929:0.5413606833758919) arc (-57.29233279583929:0.18771876786163338:0.5413606833758919);
        
        \draw [shift={(0.4963164562849324,1.2227746771979466)}] (69.84912024169617:0.40602051253191895) arc (69.84912024169617:180.18771876786164:0.40602051253191895);
        \draw [shift={(0.4963164562849324,1.2227746771979466)}] (69.84912024169617:0.3315834185677338) arc (69.84912024169617:180.18771876786164:0.3315834185677338);
        
        % \draw [shift={(3.4322447318135465,-1.7289070358702208)}] (134.8466944428081:0.4060205125319189) arc (134.8466944428081:180.18771876786164:0.4060205125319189);
        % \draw [shift={(3.4322447318135465,-1.7289070358702208)}] (134.8466944428081:0.3180494014833365) arc (134.8466944428081:180.18771876786164:0.3180494014833365);
        % \draw [shift={(5.6375557440695685,-0.7430070915455227)}] (174.33339161087738:0.7443709396418513) arc (174.33339161087738:187.10999146314168:0.7443709396418513);
        % \draw [shift={(5.6375557440695685,-0.7430070915455227)}] (174.33339161087738:0.6563998285932688) arc (174.33339161087738:187.10999146314168:0.6563998285932688);
        % \draw [shift={(5.6375557440695685,-0.7430070915455227)}] (174.33339161087738:0.5684287175446864) arc (174.33339161087738:187.10999146314168:0.5684287175446864);
        
        % \draw [shift={(0.4963164562849324,1.2227746771979466)}] (-179.81228123213836:0.47369059795390545) arc (-179.81228123213836:-134.47125690708478:0.47369059795390545);
        % \draw [shift={(0.4963164562849324,1.2227746771979466)}] (-179.81228123213836:0.385719486905323) arc (-179.81228123213836:-134.47125690708478:0.385719486905323);
        % \draw [shift={(-2.420207676157124,-1.7480815561449892)}] (7.109991463141661:0.7443709396418514) arc
        %  (7.109991463141661:19.886591315406243:0.7443709396418514);
        % \draw [shift={(-2.420207676157124,-1.7480815561449892)}] (7.109991463141661:0.656399828593269) arc (7.109991463141661:19.886591315406243:0.656399828593269);
        % \draw [shift={(-2.420207676157124,-1.7480815561449892)}] (7.109991463141661:0.5684287175446865) arc (7.109991463141661:19.886591315406243:0.5684287175446865);
        % \draw [shift={(-2.420207676157124,-1.7480815561449892)}] (0.1877187678616431:0.40602051253191895) arc (0.1877187678616431:45.5287430929152:0.40602051253191895);
        % \draw [shift={(-2.420207676157124,-1.7480815561449892)}] (0.1877187678616431:0.3180494014833365) arc (0.1877187678616431:45.5287430929152:0.3180494014833365);
        
        
        % \draw [rotate around={0.18771876786163075:(0.4904347574391314,3.0179884337769978)},very thick] (0.4904347574391314,3.0179884337769978) ellipse (7.535706036941022cm and 5.161556748282821cm);
        
        \draw [dotted] (-2.420207676157121,-1.74808155614499) circle (4.163183850649577cm);
        \draw [dotted] (3.4322447318135465,-1.7289070358702208) circle (4.163183850649577cm);
        
        
        \draw [blue, very thick] (0.4963164562849324,1.2227746771979466)-- (0.8631685296495449,2.2224933663217237);
        
        \draw [] (-2.420207676157121,-1.74808155614499)-- (3.4322447318135465,-1.7289070358702208);
        \draw [] (5.6375557440695685,-0.7430070915455227)-- (3.4322447318135465,-1.7289070358702208); 
        %     node[above, pos=0.75]{$\varepsilon$};
        \draw [] (0.4963164562849324,1.2227746771979437)-- (-2.420207676157121,-1.74808155614499);
        %     node[above left, pos=0.5]{$r$};
        \draw [] (0.4963164562849324,1.2227746771979437)-- (3.4322447318135465,-1.7289070358702208); 
        %     node[above right, pos=0.4]{$r$};
        %\draw [] (-2.420207676157121,-1.74808155614499)-- (5.6375557440695685,-0.7430070915455227);
        \draw [] (1.4947161910399636,-0.3319350635955565)-- (-2.420207676157121,-1.74808155614499);
        %     node[above, pos=0.4]{$r$};
        \draw [] (1.4947161910399636,-0.3319350635955565)-- (5.6375557440695685,-0.7430070915455227);
        %     node[above, pos=0.5]{$r$};
        \draw [] (0.4963164562849324,1.2227746771979437)-- (1.4947161910399636,-0.3319350635955565);
        
        \draw [] (-2.9430712147632248,-3.591638176924038)-- (6.270436727691272,-0.8996479592514579);
        \draw [dashed] (-1.3967761861461803,1.2165722955767182)-- (2.8257031352740394,1.2304064986960972);
        
        % \fill [black] (-2.420207676157121,-1.74808155614499) circle (2pt) 
        %     node[below] {$y_1(x)$};
        % \fill [black] (3.4322447318135465,-1.7289070358702208) circle (2pt)  
        %     node[below]{$y_2(x)$};
        \fill [blue] (0.4963164562849324,1.2227746771979437) circle (0.05);
        \fill [white] (0.7,1.4) circle (0.12);
        \node[] at (0.7,1.4) {$x$};
        \fill [blue] (1.4947161910399636,-0.3319350635955565) circle (0.05);
        \node[below] at (1.3947161910399636,-0.4319350635955565)
             {$x_\varepsilon$};
        % \fill[white] (6,-0.4430070915455227) circle (8pt);
        %\fill [black] (5.6375557440695685,-0.7430070915455227) circle (2pt)
        %     node[above]{$y_2(x_\varepsilon)$};
        
        % \node[left] at (3.1210194681658792,-1.5143221866701352) {$\alpha$};
        
        % \fill[white] (2.666203058140344,-1.7903426992020517) circle (3pt);
        % \node at (2.666203058140344,-1.7503426992020517) {$\delta$};
        % \node[left] at (4.780441689137528,-0.7534852641126851) {$\alpha_\varepsilon$};
        % \fill[white] (-0.9, -1.5739550067212016) circle (3pt);
        % \node[right] at (-1.175206169685229, -1.5839550067212016) {$\Delta$};
        \fill [blue] (0.8631685296495449,2.2224933663217237) circle (0.05)
             node[right] {$z$};
        \node at (1.75,0.95) {$\frac \pi2 - \alpha + o(1)$};
        \node at (0.25,1.75) {$\beta$};
    \end{tikzpicture}
%
%
%
%
    \hfill\phantom{}

    \caption{Нахождение координат точки $x_\varepsilon$ в случаях 3 и 4}
    \label{case34}
\end{figure}

==> pictures/rus/stadion.tex <==
\begin{figure}[h]
    \centering
 

\begin{tikzpicture}[scale=1.3]

\foreach \y in {0, 3.51389977019889} {
    \draw[very thick, loosely dotted] 
        (-1, \y) -- (0, \y);
    \draw[very thick]
        (0, \y) -- (3.66, \y);
    \draw[very thick, loosely dotted] 
        (3.66, \y) -- (4.66, \y);
}
\draw[very thick] (-1, 0) arc (270:90:1.757);
\draw[very thick] (4.66, 0) arc (-90:90:1.757);


%\draw[thin, dashed] (0.2614137092297641 + 1, 0.0) arc (0:180:1);
%\draw[thin, dashed] (0.7842411276892922 + 1, 0.0) arc (0:180:1);
%\draw[thin, dashed] (1.3070685461488205 + 1, 0.0) arc (0:180:1);
\draw[thin, dashed] (1.8298959646083486 + 1, 0.0) arc (0:180:1);
%\draw[thin, dashed] (2.3527233830678767 + 1, 0.0) arc (0:180:1);
%\draw[thin, dashed] (2.875550801527405 + 1, 0.0) arc (0:180:1);
%\draw[thin, dashed] (3.398378219986933 + 1, 0.0) arc (0:180:1);
%\draw[thin, dashed] (1.8298959646083486 + 1, 3.75) arc (0:-180:1);


\draw[blue, thick] 
(0.0, 0.9652268503449002) -- 
(1.5684822553785844, 0.9652268503449002) --
(1.8298959646083486, 1.11615412573856) --
(2.0913096738381127, 0.9652268503449002) -- 
(3.659791929216697, 0.9652268503449002);

\node[blue] at (1.61,1.8) {$\Sigma_0$};

\draw[dashed] (0.0, 0.0) -- (0.0, 3.51389977019889);
\draw[dashed] (3.659791929216697, 0.0) -- (3.659791929216697, 3.51389977019889);

\fill[blue] (0.0, 0.9652268503449002) 
    circle (1.5pt) node[black, below right] {$A$};
\fill[blue] (3.659791929216697, 0.9652268503449002) 
    circle (1.5pt) node[black, below left] {$B$};

\draw[blue, thick] 
(1.8298959646083486, 1.11615412573856) -- 
(1.8298959646083486, 2.58208251632886);

\draw[thin, dashed] (1, 3.51389977019889) arc (0:-90:1);
\draw[thin, dashed] (2.66, 3.51389977019889) arc (180:270:1);

\draw[blue, thick]
(1.8298959646083486, 2.58208251632886) -- 
(0.9149479823041743, 3.11032798020668);

\draw[blue, thick] 
(1.8298959646083486, 2.58208251632886) -- 
(2.744843946912523, 3.11032798020668);



\end{tikzpicture}

    \caption{Неоптимальность подковы для достаточно длинного стадиона с $R < 1.75r$.}
    \label{stadion}
\end{figure}
